RetinaQA: A Robust Knowledge Base Question Answering Model for both Answerable and Unanswerable Questions

An essential requirement for a real-world Knowledge Base Question Answering (KBQA) system is the ability to detect the answerability of questions when generating logical forms. However, state-of-the-art KBQA models assume all questions to be answerable. Recent research has found that such models, when superficially adapted to detect answerability, struggle to satisfactorily identify the different categories of unanswerable questions, and simultaneously preserve good performance for answerable questions. Towards addressing this issue, we propose RetinaQA, a new KBQA model that unifies two key ideas in a single KBQA architecture: (a) discrimination over candidate logical forms, rather than generating these, for handling schema-related unanswerability, and (b) sketch-filling-based construction of candidate logical forms for handling data-related unaswerability. Our results show that RetinaQA significantly outperforms adaptations of state-of-the-art KBQA models in handling both answerable and unanswerable questions and demonstrates robustness across all categories of unanswerability. Notably, RetinaQA also sets a new state-of-the-art for answerable KBQA, surpassing existing models.

==> additions.tex <==
\section{Additions}

\subsection{Terminologies}
1. Entity Linker, Sketch Generation (SG for tables), Schema Retriever (SR for tables), LF Integrator (LFI for tables), LF Retriever (LFR for tables), LF Constructor (LFC for tables), Discriminator, Thresholding, Execution Guided Check (EGC).\\

\subsection{Analysis}
Tab.~\ref{tab:num_rels_analysis} records the performance of RetinaQA for queries of different complexities represented by number of relations in s-expression (or number of hops in answer path). We can see that for 1-hop and 2-hop questions RetinaQA is better than both baselines, while for 3-hop questions RetinaQA is not the best but is better than Pangu. Further by comparing ablations i.e. without Logical Form Retriever and without (Sketch Generation and Schema Retriever) we can see that Sketch Generation and Schema Retriever contribute more to the performance of 3-hop and 4-hop questions.

\subsection{Results}
The primary focus of the paper is to propose a model robust to both answerable and unanswerable questions. Unfortunately, the only existing dataset containing both answerable and unanswerable questions is GrailQAbility. So we show experiments on two additional datasets with only answerable questions - GrailQA and WebQSP (Tab.~\ref{tab:webqsp}). The results show that the same architecture also works well for only answerable questions. 
[ TO DO : More details based on table ]

\begin{figure*}[h!]
\includegraphics[width=0.99\textwidth]{images/model_architecture_v2.png}  
\caption{
Model Architecture. Here $L$ refers to the predicted logical form and $A$ refers to the predicted answer.
}  
\label{fig:example_2}
%\vspace{-0.5cm}
\end{figure*}

\begin{table*}[h!]
\begin{center}
\small    
\begin{tabular}[b]{ccccc}
\hline
\#relation & 1 & 2  & 3 & 4 \\
% \hline
% Pangu & 82.8/87.1 & 63.5/72.4 & 24.7/45.7 & 0.0/33.3 \\
% Tiara & 73.9/79.3 & 63.2/73.3 & {\bf31.1/48.4} & {\bf50.0/76.2} \\
% RetinaQA & {\bf83.7/87.3} & {\bf68.5/76.9} & 26.9/42.8 & {\bf50.0/76.2} \\
% \hline
\hline
Pangu & 82.8 & 63.5 & 24.7 & 0.0 \\
Tiara & 81.2 & 64.7 & {\bf29.3} & {\bf50.0} \\
RetinaQA & {\bf83.7} & {\bf68.5} & 26.9 & {\bf50.0} \\
\hline
RetinaQA - LFR & 76.3 & 50.9 & 25.1 & 50.0 \\
RetinaQA - SG\_SR & 72.9 & 56.9 & 12.0 & 0.0 \\
\hline

\end{tabular}
%}
\end{center}
\caption{Performance for different types of questions on the GrailQA validation set in terms of EM. \#relation
denotes the number of relations in the s-expression.}
\label{tab:num_rels_analysis_2}
%\vspace{-0.5cm}
\end{table*}

\begin{table*}[h!]
\begin{center}
\small    
\begin{tabular}[b]{ccccc}
\hline
\#function & None & Count  & Comp. & Super.  \\
\hline
Pangu & 77.3 & 71.4 & 74.8 & {\bf72.6} \\
Tiara & 77.8 & {\bf76.4} & 57.4 & 58.7 \\
RetinaQA & {\bf79.2} & 75.5 & {\bf78.1} & 68.5 \\
\hline

\end{tabular}
%}
\end{center}
\caption{Performance for different types of questions on the GrailQA validation set in terms of EM. Function
denotes different types of function in the s-expression - none, count, comperative and superlative.}
\label{tab:func_analysis}
%\vspace{-0.5cm}
\end{table*}


\iffalse
\begin{table*}[h!]
\begin{center}
\small    
\begin{tabular}[b]{|c|c|}
\hline
\#model & F1 \\
\hline
Tiara & {\bf75.8} \\
Pangu & 70.6 \\
RetinaQA & 74.7 \\
\hline

\end{tabular}
%}
\end{center}
\caption{Results on WebQSP-test set}
\label{tab:webqsp}
%\vspace{-0.5cm}
\end{table*}
\fi


\subsection{Examples}

1. Known logical form
    a. No incompletness : Can add example similar to 2.
    b. Data incompletness (in current model architecture) 

2. L = NK \\
    \fbox{\begin{minipage}{32em}
    \textbf{question} : In which conference is Glove published?\\
    \textbf{$L^{\ast}$} : (AND Conference (JOIN (R published at) Glove))\\
    \textbf{Missing KB element} : published at \\
    \textbf{Entity Linker Output} : Glove \\
    \textbf{Sketch Generation Output} : (AND type (JOIN R relation entity)) \\
    \textbf{schema retriever output} : \\top\_types : Publisher, Conference,  top\_relations : is written, presented at\\
     \textbf{LF integrator output} : (AND Conference (JOIN R is written Glove)), (AND Publisher (JOIN R presented at Glove))\\
    \textbf{LF retriever output} : (AND Researcher (JOIN writes Glove)) , (COUNT (AND Researcher (JOIN writes Glove)))
    \textbf{Discriminator output} : (AND Researcher (JOIN writes Glove)) , score = 0.03 \\
    \textbf{Thresholding output} : NK
    \textbf{answer} : \text{[NA]}
    \end{minipage}}

==> checklist.tex <==

A. For every submission:\\
A1. Did you describe the limitations of your work? {\bf Yes.}\\
%Point out any strong assumptions and how robust your results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only held locally). Reflect on how these assumptions might be violated in practice and what the implications would be.
%Reflect on the scope of your claims, e.g., if you only tested your approach on a few datasets, languages, or did a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated. Reflect on the factors that influence the performance of your approach. For example, a speech-to-text system might not be able to be reliably used to provide closed captions for online lectures because it fails to handle technical jargon.
%If you analyze model biases: which definition of bias are you using? Did you state the motivation and definition explicitly? See the discussion in Blodgett et al. (2020).
%We understand that authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection. It is worth keeping in mind that a worse outcome might be if reviewers discover limitations that aren’t acknowledged in the paper. In general, we advise authors to use their best judgement and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
A2. Did you discuss any potential risks of your work? {\bf Yes}\\
%Examples of risks include potential malicious or unintended harmful effects and uses (e.g., disinformation, generating fake profiles, surveillance), environmental impact (e.g., training huge models), fairness considerations (e.g., deployment of technologies that could further disadvantage or exclude historically disadvantaged groups), privacy considerations (e.g., a paper on model/data stealing), and security considerations (e.g., adversarial attacks). See discussion in Leins et. al. (2020) as examples.
%Does the research contribute to overgeneralization, bias confirmation, under or overexposure of specific languages, topics, or applications at the expense of others? See Hovy and Spruit (2016) for examples.
%We expect many papers to be foundational research and not tied to particular applications, let alone deployments. However, we encourage authors to discuss potential risks if they see a path to any positive or negative applications. For example, the authors can emphasize how their systems are intended to be used, how they can safeguard their systems against misuse, or propose future research directions.
%Consider different stakeholders that could be impacted by your work. Is it possible that research benefits some stakeholders while harming others? Does it pay special attention to vulnerable or marginalized communities? Does the research lead to exclusion of certain groups? See Dev et. al (2021) for examples.
%Consider dual use, i.e, possible benefits or harms that could arise when the technology is being used as intended and functioning correctly, benefits or harms that could arise when the technology is being used as intended but gives incorrect results, and benefits or harms following from (intentional or unintentional) misuse of the technology.
%Consider citing previous work on relevant mitigation strategies for the potential risks of the work (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of NLP).
A3. Do the abstract and introduction summarize the paper’s main claims? {\bf Yes}\\
%The main claims in the paper should be clearly stated in the abstract and in the introduction.
%These claims should be supported by evidence presented in the paper, potentially in the form of experimental results, reasoning, or theory. The connection between which evidence supports which claims should be clear.
%The context of the contributions of the paper should be clearly described, and it should be stated how much the results would be expected to generalize to other contexts.
%It should be easy for a casual reader to distinguish between the contributions of the paper and open questions, future work, aspirational goals, motivations, etc.
B. Did you use or create scientific artifacts? {\bf Yes}\\
%Scientific artifacts may include code, data, models or other artifacts.
%Most NLP research uses scientific artifacts.
%Many NLP papers are accompanied by new scientific artifacts.
B1. Did you cite the creators of artifacts you used? {\bf Yes}\\
%For composite artifacts like the GLUE benchmark, this means all creators.
%Cite the original paper that produced the code package or dataset.
%Remember to state which version of the asset you’re using.
%If possible, include a URL.
B2. Did you discuss the license or terms for use and / or distribution of any artifacts?\\
%State the name of the license (e.g., CC-BY 4.0) for each asset.
%If you scraped or collected data from a particular source (e.g., website or social media API), you should state the copyright and terms of service of that source. Please note that some sources do not allow inference of protected categories like gender, sexual orientation, health status, etc.
%The data might be in public domain and licensed for research purposes.
%The data might be used with consent of its creators or copyright holders.
%If the data is used without consent, the paper makes the case to justify its legal basis (e.g., research performed in the public interest under GDPR).
%If you are releasing assets, you should include a license, copyright information, and terms of use in the package.
%If you are repackaging an existing dataset, you should state the original license as well as the one for the derived asset (if it has changed).
%If you cannot find this information online, you are encouraged to reach out to the asset’s creators.
B3. Did you discuss if your use of existing artifact(s) was consistent with their intended use, provided that it was specified? For the artifacts you create, do you specify intended use and whether that is compatible with the original access conditions (in particular, derivatives of data accessed for research purposes should not be used outside of research contexts)? {\bf Yes}\\
%Data and/or pretrained models are released under a specified license that is compatible with the conditions under which access to data was granted (in particular, derivatives of data accessed for research purposes should not be deployed in the real world as anything other than a research prototype, especially commercially)
%The paper specifies the efforts to limit the potential use to circumstances in which the data/models could be used safely (such as an accompanying data/model statement).
%The data is sufficiently anonymized to make identification of individuals impossible without significant effort. If this is not possible due to the research type, please state so explicitly and explain why.
%The paper discusses the harms that may ensue from the limitations of the data collection methodology, especially concerning marginalized/vulnerable populations, and specifies the scope within which the data can be used safely.
B4. Did you discuss the steps taken to check whether the data that was collected / used contains any information that names or uniquely identifies individual people or offensive content, and the steps taken to protect / anonymize it? {\bf NA.}\\
%There are some settings where the existence of offensive content is not necessarily bad (e.g., swear words occur naturally in text), or part of the research question (i.e., hate speech). This question is just to encourage discussion of potentially undesirable properties.
%Explain how you checked for offensive content and identifiers (e.g., with a script, manually on a sample, etc.).
%Explain how you anonymized the data, i.e., removed identifying information like names, phone and credit card numbers, addresses, user names, etc. Examples are monodirectional hashes, replacement, or removal of data points. If anonymization is not possible due to the nature of the research (e.g., author identification), explain why.
%List any further privacy protection measures you are using: separation of author metadata from text, licensing, etc.
%If any personal data is used: the paper specifies the standards applied for its storage and processing, and any anonymization efforts.
%If the individual speakers remain identifiable via search: the paper discusses possible harms from misuse of this data, and their mitigation.
B5. Did you provide documentation of the artifacts, e.g., coverage of domains, languages, and linguistic phenomena, demographic groups represented, etc.? {\bf NA}\\
%Be sure to report the language of any language data, even if it is commonly-used benchmarks.
%Describe basic information about the data that was used, such as the domain of the text, any information about the demographics of the authors, etc.
B6. Did you report relevant statistics like the number of examples, details of train / test / dev splits, etc. for the data that you used / created? {\bf Yes}\\
%Even for commonly-used benchmark datasets, include the number of examples in train / validation / test splits, as these provide necessary context for a reader to understand experimental results. For example, small differences in accuracy on large test sets may be significant, while on small test sets they may not be.\\
C. Did you run computational experiments? {\bf Yes}\\
C1. Did you report the number of parameters in the models used, the total computational budget (e.g., GPU hours), and computing infrastructure used? {\bf Yes}\\
%Even for commonly-used models like BERT, reporting the number of parameters is important because it provides context necessary for readers to understand experimental results. The size of a model has an impact on performance, and it shouldn’t be up to a reader to have to go look up the number of parameters in models to remind themselves of this information.
%The total computational budget can be presented however is most appropriate for the paper – if most experiments were run on GPUs, then important information would likely include the total number of GPU hours, the amount of parallelism across GPUs, the size of the GPUs, etc. to allow a reader to estimate the computational requirements to reproduce, use, or build upon the work.
%Note that this should include information about all experiments, not just the final runs that led to the results presented in the paper. If exact numbers are not available, an estimate is better than nothing.
C2. Did you discuss the experimental setup, including hyperparameter search and best-found hyperparameter values? {\bf Yes}\\
%The experimental setup should include information about exactly how experiments were set up, like how model selection was done (e.g., early stopping on validation data, the single model with the lowest loss, etc.), how data was preprocessed, etc.
%Many research projects involve manually tuning hyperparameters until some “good” values are found, and then running a final experiment which is reported in the paper. Other projects involve using random search or grid search to find hyperparameters. In all cases, report the results of such experiments, even if they were stopped early or didn’t lead to your best results, as it allows a reader to know the process necessary to get to the final result and to estimate which hyperparameters were important to tune.
%Be sure to include the best-found hyperparameter values (e.g., learning rate, regularization, etc.) as these are critically important for others to build on your work.
%The experimental setup should likely be described in the main body of the paper, as that is important for reviewers to understand the results, but large tables of hyperparameters or the results of hyperparameter searches could be presented in the main paper or appendix.
C3. Did you report descriptive statistics about your results (e.g., error bars around results, summary statistics from sets of experiments), and is it transparent whether you are reporting the max, mean, etc. or just a single run? {\bf Yes}\\
%Error bars can be computed by running experiments with different random seeds, Clopper–Pearson confidence intervals can be placed around the results (e.g., accuracy), or expected validation performance can be useful tools here.
%In all cases, when a result is reported, it should be clear if it is from a single run, the max across N random seeds, the average, etc.
%When reporting a result on a test set, be sure to report a result of the same model on the validation set (if available) so others reproducing your work don’t need to evaluate on the test set to confirm a reproduction.
C4. If you used existing packages (e.g., for preprocessing, for normalization, or for evaluation), did you report the implementation, model, and parameter settings used (e.g., NLTK, Spacy, ROUGE, etc.)? {\bf Yes}\\
%The version number or reference to specific implementation is important because different implementations of the same metric can lead to slightly different results (e.g., ROUGE).
%The paper cites the original work for the model or software package. If no paper exists, a URL to the website or repository is included.
%If you modified an existing library, explain what changes you made.
D. Did you use human annotators (e.g., crowdworkers) or research with human participants? {\bf No.}\\
%D1. Did you report the full text of instructions given to participants, including e.g., screenshots, disclaimers of any risks to participants or annotators, etc.?\\
%Examples of risks include a crowdsourcing experiment which might show offensive content or collect personal identifying information (PII). Ideally, the participants should be warned.
%Including this information in the supplemental material is fine, but if the main contribution of your paper involves human subjects, then we strongly encourage you to include as much detail as possible in the main paper.
%D2. Did you report information about how you recruited (e.g., crowdsourcing platform, students) and paid participants, and discuss if such payment is adequate given the participants’ demographic (e.g., country of residence)?\\
%Be explicit about how you recruited your participants. For instance, mention the specific crowdsourcing platform used. If participants are students, give information about the population (e.g., graduate/undergraduate, from a specific field), and how they were compensated (e.g., for course credit or through payment).
%In case of payment, provide the amount paid for each task (including any bonuses), and discuss how you determined the amount of time a task would take. Include discussion on how the wage was determined and how you determined that this was a fair wage.
%D3. Did you discuss whether and how consent was obtained from people whose data you’re using/curating? For example, if you collected data via crowdsourcing, did your instructions to crowdworkers explain how the data would be used?\\
%D4. Was the data collection protocol approved (or determined exempt) by an ethics review board?\\
%Depending on the country in which research is conducted, ethics review (e.g., from an IRB board in the US context) may be required for any human subjects research. If an ethics review board was involved, you should clearly state it in the paper. However, stating that you obtained approval from an ethics review board does not imply that the societal impact of the work does not need to be discussed.
%For initial submissions, do not include any information that would break anonymity, such as the institution conducting the review.
%D5. Did you report the basic demographic and geographic characteristics of the annotator population that is the source of the data?\\
%State if your data include any protected information (e.g., sexual orientation or political views under GDPR).
%The paper is accompanied by a data statement (see Bender and Friedman, 2018) describing the basic demographic and geographic characteristics of the author population that is the source of the data, and the population that it is intended to represent.
%If applicable: the paper describes whether any characteristics of the human subjects were self-reported (preferably) or inferred (in what way), justifying the methodology and choice of description categories.


==> task.tex <==
\section{KBQA with Answerability Detection}
\label{sec:task}

%We first introduce the notion of unanswerable KG questions and different ways of training to detect answerability, and then introduce a new benchmark dataset for KG-QA with answerable questions.

\iffalse 
\begin{figure}[t]
\centering
\includegraphics[width=0.95\columnwidth]{images/incompletnessKG.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
  \caption{Types of Incompleteness in KG}
  \label{fig:incompletness_KG}
  %\vspace{-0.5cm}
\end{figure}
\fi

A {\em Knowledge Base} (KB) (also called Knowledge Graph) $G$ contains a {\em schema} $S$ (or ontology) with {\em entity types} (or types) $T$ and {\em relations} $R$ defined over pairs of types, which we together refer to as {\em schema elements} of the KB.
The types in $T$ are often organized as a hierarchy.
It also contains {\em entities} $E$ as instances of types, and {\em facts} (or triples) $F\subseteq E \times R \times E$, which we together refer to as {\em data elements} of the KB.
%(A KB also contains literals, which we ignore for brevity of notation.)
The top layer of Fig.~\ref{fig:example}(A) shows example schema elements, while the bottom layer shows entities and facts.
In {\em Knowledge Base Question Answering} (KBQA), we are given a {\em question} $q$ written in natural language which needs to be translated to a {\em logical form} (or query) $l$ that executes over $G$ to yield a set of {\em answers} $A$.
%Since a question may have many answers, $a$ is a set.
%{\color{red}
Different logical forms, SPARQL~\cite{webqsp}, s-expressions~\cite{gu:www2021grailqa}, programs~\cite{KQAPro}, etc., have been used in the KBQA literature.
%}
We concentrate on {\em s-expressions}~\cite{gu:www2021grailqa}, 
which employ set-based semantics and functions with arguments and return values as sets.
These can be easily translated to KB query languages such as SPARQL, and provide a balance between readability and compactness~\cite{gu:www2021grailqa}.
We call a logical form {\em valid} for $G$ if it executes over $G$ without an error.
On successful execution, a logical form traces a {\em path} in the KB leading to each answer.
Fig.~\ref{fig:example}(A) shows an example query with a valid logical form (using s-expression) and the path traced by its execution.
%When a query has multiple answers, it has a corresponding path for each answer.

%In Fig.~\ref{fig:example}, we illustrate answerable and different forms of unanswerable questions.
We define a question $q$ to be {\bf answerable} for a KB $G$, if {\bf (a)} $q$ admits a valid logical form $l$ for $G$, AND {\bf (b)} $l$ returns a {\em non-empty} answer set $A$ when executed over $G$.
The example question in Fig.~\ref{fig:example}(A) is answerable for the shown KB.
%Note that this definition does not address correctness or completeness of the facts in $G$ and therefore of the answer.
The \emph{standard} KBQA task over a KB $G$ is to output the answer $A$, and optionally the logical form $l$, given a question $q$, {\em assuming $q$ to be answerable for $G$}.

Most recent KBQA models~\cite{ye:acl2022rngkbqa,chen:acl2021retrack} are trained with questions and gold logical forms.
Other models directly generate the answer~\cite{sun-etal-2019-pullnet,saxena:acl2022seq2seqembedkgqa}.
Different train-test settings
% --- IID, zero-shot and compositional generalization --- 
have been explored and are included in benchmark KBQA datasets~\cite{gu:www2021grailqa}.
For a question $q$, let $S_q$ denote the schema elements in the logical form for $q$.
Given a training set $Q_{tr}$, a test question $q$ is labelled {\em IID} if it follows the distribution for questions in $Q_{tr}$, and contains only schema elements seen in train $S_q\subseteq S_{Q_{tr}}$ (we have overloaded notation to define $S_{Q_{tr}}$).
Alternatively, a test question $q$ is labelled {\em zero shot} if it involves at least one unseen schema element ($S_q\not \subseteq S_{Q_{tr}}$).
Finally, test question $q$ involves {\em compositional generalization} if $S_q\subseteq S_{Q_{tr}}$ but the specific logical form for $q$ does not match that for any $q'\in Q_{tr}$.

%A question in KG-QA is answerable when all relevant schema (Entity Type/Class and Relationships) and data (entities and facts) items are present in the KG, for e.g., Q1 in Fig. \ref{fig:incompletness_KG}. So a question in KG-QA becomes unanswerable due to missing data items i.e., facts(Q2 and Q3), entity (Q4) or schema items i.e., relationships (Q5), entity Types (Q6), and their combination. Missing data items only affect specific questions whereas missing schema items affect an entire class of questions i.e., the logical form is no longer valid for questions (Q4, Q5, and Q6) where corresponding schema items or mentioned entities are missing from the KG.  

\iffalse
 \begin{figure}[t]
\centering
\includegraphics[width=0.95\columnwidth]{images/train_test_generalisation.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
  \caption{Different levels of generalization for answerable and unanswerable questions}
  \label{fig:generalisation}
  %\vspace{-0.5cm}
\end{figure}
\fi

By negating the above answerability definition, we define a question $q$ to be {\bf unanswerable} for a KB $G$ if {\bf (a)} $q$ does not admit a valid logical form $l$ for $G$, or {\bf (b)} the valid $l$ when executed over the $G$ returns an empty answer. 
Clearly, meaningless and out-of-scope questions for a KB are unanswerable.
Even for a meaningful question, unanswerability arises due to incompleteness (in data or schema) in $G$.
Such questions admit an `ideal KB' $G^*$ for which $q$ has a valid ideal logical form $l^*$ which executes on $G^*$ to generate a non-empty ideal answer $a^*$. 
The available KB $G$ lacks one or more schema or data elements making $q$ unanswerable.
Fig.~\ref{fig:example}(A) illustrates an available KB, with missing elements with respect to the ideal KB shown in red.
In Fig.~\ref{fig:example}(B), questions 1-2 yield valid queries for the available KB but missing facts lead to empty answers, while questions 3-5 lack schema elements for valid queries.

The task of {\bf KBQA with answerability detection}, given a question $q$ and an available KB $G$, is to {\bf (a)} appropriately label the answer $A$ as $\mbox{NA}$ (No Answer) or the logical form $l$ as $\mbox{NK}$ (No Knowledge, i.e., query not possible) when $q$ is unanswerable for $G$, or {\bf (b)} generate the correct non-empty answer $A$ and valid logical form $l$ when $q$ is answerable for $G$.
%(For models that directly generate the answer, $l$ may be left out.)
%requires labeling a given question as {\bf NK} (denoting no knowledge) or {\bf NA} (denoting no answer) or generating an answer.
%Optionally, the logical form, when it exists, can be generated in place of the answer.
%During test, the task is to predict the logical form when it exists and NK otherwise, and further the answer when it exists and NA otherwise.
%Note that the second task is addressed by the query engine and is thus beyond the KG-QA system, and thus the task primarily involves predicting a logical form or NK for a given question.
The training set may now additionally include unanswerable questions labeled appropriately with $A=\mbox{NA}$ or $l=\mbox{NK}$.
Note that training instances do not contain `ideal' logical forms for the unanswerable questions that have $l=\mbox{NK}$.
%These are labeled with {\bf NK} (denoting no knowledge) when the logical form does not exist for the KG, or with {\bf NA} (denoting no answer) when the logical form exists but the KG does not have any answers.
%Note that the ideal logical form (for a complete KG) is not provided for NK questions.

Mirroring answerable questions, we define different train-test scenarios for unanswerable questions as well. %which we call {\em IID}, {\em full zero-shot} and {\em partial zero-shot}.
An {\em IID unanswerable} question in test follows the same distribution as unanswerable questions in train, and all missing KB elements (schema elements in its ideal logical form 
%{\color{red}
and missing data elements in its ideal paths)
are encountered in train unanswerable questions associated with the same category of incompleteness.
%}
For example, the missing schema element {\em Research Area} for the first test question in Fig.~\ref{fig:example}(C) is covered by the second train question.
%For an IID NA test question, all `missing' KG elements (entity type or relation) in its `ideal logical form' are `seen' in the ideal logical form of some training question labeled NK.  
In contrast, a {\em zero-shot unanswerable test question} involves at least one missing KB element (schema element in its ideal logical form or data element in its paths) that is not part of any unanswerable question in train associated with same category of incompleteness.
E.g., the missing schema elements ({\em located in} and {\em works at}) for the second and third test questions in Fig.\ref{fig:example}(C) are not covered by any unanswerable question in train.
%are generated from a different distribution over unanswerable questions than that in train. 
%The ideal logical form for these questions contains at least one `unseen missing' schema element --- one that does not appear in the ideal logical form of any unanswerable question in train. 
%Such questions are expected to form a large fraction of unanswerable questions in test sets from real KBQA applications. 
%However, differently from answerable questions, ideal logical forms containing missing schema elements are {\em not provided} for training - these are only labeled as $\mbox{NK}$.
%If all of the schema elements in the ideal logical form are `unseen missing', then we term it {\em full zero-shot}. 
%Otherwise, if the ideal logical form contains both seen KB elements from answerable train questions and unseen missing KB elements, we term it {\em partial zero-shot}.
%Note that KBQA datasets do not make this distinction for answerable questions.
%For unanswerable questions, our experiments show that these are not equally difficult.
We further define two sub-classes, partial and complete zero-shot, for zero-shot unanswerable questions, but for clarity, discuss these in Sec. \ref{sec:results}.

%Answering an i.i.d question can be achieved with memorization without requiring  generalization because, for a test question, the KGQA model has to predict the logical form seen during training with a different instantiation of schema items for e.g., questions \textit{Tr1} and \textit{Te1} in Fig. \ref{fig:generalisation}. A harder setting is when a novel combination of seen schema items is required to answer a question i.e., compositional generalisation, for e.g., \textit{Tr3} and \textit{Te2} in Fig. \ref{fig:generalisation}. And even a harder setting is when one or more schema items unseen  during training are required to answer a given question i.e., zero-shot generalization for e.g., \textit{{Te3}} in Fig. \ref{fig:generalisation}.  
%Similar to answerable i.i.d questions, we define unanswerable i.i.d questions where an unanswerable question in train and test share the same type of KG incompleteness for e.g., \textit{{Tr2}} and \textit{Te4}  in Fig. \ref{fig:generalisation}.
%Detecting such unanswerability can be achieved with memorization without requiring generalization. So to make answerability detection more challenging, similar to zero-shot answerable, we also introduce two types of zero-shot unanswerable questions i.e., zero-shot complete and zero-shot partial. Schema items corresponding to zero-shot complete unanswerable questions are missing from the corresponding logical form whereas for zero-shot partial unanswerable questions atleast one schema item that is seen during training is present in the KG. \textit{Te5} and \textit{Te6} are examples of zero-shot partial and zero-shot complete unanswerable questions respectively, in Fig. \ref{fig:generalisation}.

%In GrailQA dataset, KGQA model trained on answerable questions is expected to answer i.i.d questions along with questions where KGQA model has to generate a logical form consisting of a novel composition of seen schema items during training i.e., compositional generalization and logical form with at least one unseen schema item during the training in case of zero-shot generalization.

%\textbf{Different levels of generalization in answerable and unanswerable questions....}

